Design and Numerical Analysis of Hyperbolic Metamaterial Based Ultrasensitive E. Coli Sensor

We proposed an extremely sensitive \textit{E. Coli} sensor based on a hyperbolic metamaterial structure combining ultra-thin Ag-Al$_2$O$_3$ layers to minimize metallic optical loss. The principle relied on detecting the change in the resonance wavelength due to the interaction of bacteria with the surrounding aqueous environment by utilizing the finite-difference time-domain numerical technique. Our proposed hyperbolic metamaterial \textit{E. Coli} sensor operated in the range from visible to near-infrared wavelengths exhibiting strong bulk plasmon polaritons at the hyperbolic regime ($\lambda \geq$ 460 nm). An anisotropic hyperbolic range was obtained theoretically by solving the effective medium theory. An outstanding sensitivity of 9000 nm per bacteria was achieved for a bulk plasmon-polariton mode. The hyperbolic metamaterial was the origin of obtaining such extremely high sensitivity; no bulk plasmon polaritons were found without hyperbolic metamaterial. We analyzed the effect of different shapes in two-dimensional Ag differential grating on sensing performance. Additionally, we compared the performance parameters of our proposed \textit{E. Coli} sensor with recently demonstrated sensors. Our proposed hyperbolic metamaterial structure has the potential as a highly sensitive \textit{E. Coli} sensor operating in a wide range of wavelengths for label-free detection.

==> table.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[htbp]
\caption{Comparative performance analysis of biosensors}
\begin{center}

\begin{tabular}{c c c c c}
\hline
Structure & Wavelength ($\mu$m) & Sensitivity &  Q-factor & Ref. \\
\hline
Triangular gold nanoparticles & 0.5 -- 0.7 & $<$110.7 nm/mM & $<$ 2.92 & \cite{Chowdhury} \\

Au/1D photonic crystal & 0.6 -- 0.8 & 53.5 nm/RIU & $<$ 0.69 & \cite{Ahmed} \\

Double spilt-ring resonator & 150 -- 300 & 387 GHz/RIU & -- & \cite{Nine} \\ 

Graphene/MoS2 crumpled sensor & 4 -- 10 & 7499 nm/RIU & 67 & \cite{vahid} \\

Ag-Al$_2$O$_3$ HMM sensor & 0.5 -- 2.0 & 9000 nm/bacteria & 107.6 & This work \\
\hline
\end{tabular}
\label{Tab:1}
\end{center}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%
